Probing Cross-modal Semantics Alignment Capability from the Textual Perspective

In recent years, vision and language pre-training (VLP) models have advanced the state-of-the-art results in a variety of cross-modal downstream tasks. Aligning cross-modal semantics is claimed to be one of the essential capabilities of VLP models. However, it still remains unclear about the inner working mechanism of alignment in VLP models. In this paper, we propose a new probing method that is based on image captioning to first empirically study the cross-modal semantics alignment of VLP models. Our probing method is built upon the fact that given an image-caption pair, the VLP models will give a score, indicating how well two modalities are aligned; maximizing such scores will generate sentences that VLP models believe are of good alignment. Analyzing these sentences thus will reveal in what way different modalities are aligned and how well these alignments are in VLP models. We apply our probing method to five popular VLP models, including UNITER, ROSITA, ViLBERT, CLIP, and LXMERT, and provide a comprehensive analysis of the generated captions guided by these models. Our results show that VLP models (1) focus more on just aligning objects with visual words, while neglecting global semantics; (2) prefer fixed sentence patterns, thus ignoring more important textual information including fluency and grammar; and (3) deem the captions with more visual words are better aligned with images. These findings indicate that VLP models still have weaknesses in cross-modal semantics alignment and we hope this work will draw researchers' attention to such problems when designing a new VLP model.

==> tables/tb-ic_metrics.tex <==

% \begin{table*}[h!]
% % \resizebox{0.49\textwidth}{!}{
% \centering
% \small
% \begin{tabular}{lcccccc}
% \toprule
% \textbf{Model} & \textbf{Bleu1} & \textbf{Bleu4} & \textbf{METEOR} & \textbf{ROUGE} & \textbf{CIDEr} & \textbf{SPICE} \\
% \midrule
% UNITER & 44.5 & 6.0 & 14.3 & 35.8 & 34.9 & 9.7  \\
% ViLBERT & 23.8 & 2.2 & 13.5 & 23.7 & 6.6 & 12.0 \\
% CLIP & 31.2 & 3.9 & 16.4 & 31.0 & 10.3 & 10.3 \\
% ROSITA & 25.2 & 1.0 & 13.8 & 26.7 & 5.3 & 9.1 \\
% LXMERT & 30.0 & 3.3 & 16.1 & 31.2 & 9.3 & 11.3 \\
% \midrule
% CE & 72.2 & 28.7 & 24.4 & 52.4 & 92.0 & 17.4 \\
% \bottomrule
% \end{tabular}
% % }
% \caption{Results of various VLP models on image captioning metrics. Except the CE model, other models are trained under SCST framework.}
% \label{tb:rl_results}
% \end{table*}

==> tables/tb-nouns.tex <==

\begin{table}[h!]
\centering
% \begin{tabular}{p{2.5cm}lp{1.5cm}cp{1.5cm}c}
\resizebox{0.49\textwidth}{!}{
\begin{tabular}{lccccc}
\toprule 
\diagbox {\textbf{Model}} {\textbf{Number}} & \textbf{3} & \textbf{4} & \textbf{5} & \textbf{6} & \textbf{7}\\\midrule

UNITER & 79.8 & 82.7 & 83.7 & 85.2 & 86.2 \\\midrule
ROSITA & 93.1 & 93.1 & 94.4 & 94.6 & 94.2 \\\midrule
ViLBERT & 82.3 & 86.2 & 89.2 & 90.8 & 91.8 \\\midrule
CLIP & 28.1 & 29.0 & 29.7 & 30.1 & 30.3 \\\midrule
LXMERT & 81.9 & 85.7 & 88.2 & 89.8 & 90.0 \\

\bottomrule
\end{tabular}
}
\caption{Results of the effect of VLP models with the number of nouns increasing}

\label{tb:nouns}
\end{table}


==> tables/tb-replace_result.tex <==

\begin{table}[h!]
\centering
% \begin{tabular}{p{2.5cm}lp{1.5cm}cp{1.5cm}c}
\resizebox{0.49\textwidth}{!}{
\begin{tabular}{lccc}
\toprule 
\textbf{Model} & \textbf{CE} & \textbf{Replace others} & \textbf{Replace nouns} \\\midrule

UNITER & 71.6 & 63.3 &  15.4 \\\midrule
ROSITA & 86.5 & 74.1 &  49.0\\\midrule
ViLBERT & 84.6 & 83.8 &  36.8\\\midrule
CLIP & 27.8 & 24.7 &  19.6 \\\midrule
LXMERT & 80.1 & 80.0 &  40.5\\

\bottomrule
\end{tabular}
}
\caption{\maz{change to line chart.}}

\label{tb:verify_nouns}
\end{table}



